Graph-Based Continual Learning

Despite significant advances, continual learning models still suffer from catastrophic forgetting when exposed to incrementally available data from non-stationary distributions. Rehearsal approaches alleviate the problem by maintaining and replaying a small episodic memory of previous samples, often implemented as an array of independent memory slots. In this work, we propose to augment such an array with a learnable random graph that captures pairwise similarities between its samples, and use it not only to learn new tasks but also to guard against forgetting. Empirical results on several benchmark datasets show that our model consistently outperforms recently proposed baselines for task-free continual learning.

==> tables/accuracy-epoch.tex <==
\begin{table}[H]
    \caption{\small Classification results ($\%$) on \textsc{Split CIFAR100} with different number of epochs. When used, episodic memories contain 5 samples per class on average. The symbol $\uparrow$ ($\downarrow$) indicates that a higher (lower) number is better.}
    \centering
    \begin{small}
        \begin{tabular}{l@{\hskip 0.15in}r@{\hskip 0.15in}r@{\hskip 0.15in}r@{\hskip 0.15in}r@{\hskip 0.15in}r@{\hskip 0.15in}r}
            \toprule
            \textsc{Training} & \multicolumn{2}{c}{\textsc{1 epoch}} & \multicolumn{2}{c}{\textsc{10 epochs}}                                                           \\
            \cmidrule(r){1-1} \cmidrule(r){2-3} \cmidrule(r){4-5}
            Method            & \textsc{ACC} $(\uparrow)$            & \textsc{FGT} $(\downarrow)$            & \textsc{ACC} $(\uparrow)$ & \textsc{FGT} $(\downarrow)$ \\
            \midrule
            Finetune          & 47.47 $\pm$ 2.77                     & 10.94 $\pm$ 2.29                       & 55.39 $\pm$ 1.94          & 25.94 $\pm$ 1.89            \\
            EWC               & 48.39 $\pm$ 0.99                     & 6.49 $\pm$ 1.28                        & 55.60 $\pm$ 1.11          & 23.53 $\pm$ 1.19            \\
            \midrule
            ICARL             & 52.18 $\pm$ 0.27                     & 8.63 $\pm$ 2.71                        & 58.74 $\pm$ 0.74          & 9.02 $\pm$ 2.49             \\
            GEM               & 57.90 $\pm$ 1.13                     & 7.51 $\pm$ 1.52                        & 65.66 $\pm$ 0.70          & 15.52 $\pm$ 0.41            \\
            ER                & 65.61 $\pm$ 1.28                     & 5.05 $\pm$ 2.23                        & 69.40 $\pm$ 1.21          & 11.25 $\pm$ 1.24            \\
            \textbf{GCL}      & \textbf{69.82} $\pm$ 1.05            & \textbf{4.27} $\pm$ 2.35               & \textbf{74.51} $\pm$ 0.99 & \textbf{6.54} $\pm$ 1.26    \\
            \bottomrule
        \end{tabular}
    \end{small}
    \label{table:split-cifar100-epochs}
\end{table}
